Cross-Care: Assessing the Healthcare Implications of Pre-training Data on Language Model Bias

Large language models (LLMs) are increasingly essential in processing natural languages, yet their application is frequently compromised by biases and inaccuracies originating in their training data. In this study, we introduce Cross-Care, the first benchmark framework dedicated to assessing biases and real world knowledge in LLMs, specifically focusing on the representation of disease prevalence across diverse demographic groups. We systematically evaluate how demographic biases embedded in pre-training corpora like $ThePile$ influence the outputs of LLMs. We expose and quantify discrepancies by juxtaposing these biases against actual disease prevalences in various U.S. demographic groups. Our results highlight substantial misalignment between LLM representation of disease prevalence and real disease prevalence rates across demographic subgroups, indicating a pronounced risk of bias propagation and a lack of real-world grounding for medical applications of LLMs. Furthermore, we observe that various alignment methods minimally resolve inconsistencies in the models' representation of disease prevalence across different languages. For further exploration and analysis, we make all data and a data visualization tool available at: www.crosscare.net.

==> archive/2_related_work_old.tex <==
\subsection{Language model biases arise from pre-training data}
The sheer breadth of data sources consumed by such models enables the emergence of impressive capabilities across a wide range of tasks. However, this expansive data consumption has its pitfalls, as while LLM performance generally improves as models are scaled, this improvement is not uniformly distributed across all domains \cite{magnusson2023paloma}. Furthermore, it can lead to the phenomenon of 'bias exhaust'—the inadvertent propagation of biases present in the pretraining data. The propensity of language models to inherit and perpetuate societal biases observed in their training datasets is a well-documented concern in current large language model (LLM) training methodologies \cite{webster2021measuring, kaneko2021unmasking, zack2024assessing, gallifant2024peer, omiye2023large}. Efforts to mitigate this issue through the careful selection of 'clean' data have demonstrated a significant reduction in toxicity and biases \cite{li2023textbooks, biderman2023pythia}, underscoring the crucial link between the choice of pretraining corpora and the resultant behaviors of the models. Furthermore, recent studies have further elucidated the impact of pretraining data selection on the manifestation of political biases at the task level \cite{feng2023pretraining}. 

\subsection{Language model biases evaluation}
The evaluation of biases in NLP has evolved to distinguish between intrinsic and extrinsic assessments\cite{lum2024bias}. Intrinsic evaluations focus on the inherent properties of the model, while extrinsic evaluations measure biases in the context of specific tasks. This distinction has become increasingly blurred with advancements in language modeling, such as fine-tuning and in-context learning, expanding the scope of what is considered "intrinsic" \cite{goldfarbtarrant2021intrinsic}.

In the era of static word embedding models, such as word2vec \cite{mikolov2013efficient} and fastText \cite{bojanowski-etal-2017-enriching}, intrinsic evaluations were confined to metrics over the embedding space. Early examples of intrinsic bias metrics include the approach by Bolukbasi et al. \cite{Bolukbasi2016ManIT}, aggregating cosine similarity measures between words associated with different identity groups and words in a domain of interest, such as occupations. In contrast, extrinsic evaluations measured bias in models that utilized these embeddings for coreference resolution and hate speech detection tasks.

Unlike static word embedding models, LLMs feature dynamic embeddings that change with context and are inherently capable of next-word prediction, a task that can be applied to numerous objectives. To evaluate bias in LLMs, Guo, and Caliskan \cite{GuoCaliskan2021EmergentBiases} developed the Contextualized Embedding Association Test (CEAT), an extension of WEAT. Other intrinsic metrics for LLMs include StereoSet \cite{nadeem2020stereoset} and ILPS \cite{kurita2019measuring}, which are based on the log probabilities of words in text that can evoke stereotypes.

Probability-based bias evaluations such as CrowS-Pairs \cite{nangia2020crowspairs} and tasks in the BIG-bench benchmarking suite \cite{srivastava2023imitation} compare the probabilities of stereotype-related tokens conditional on the presence of identity-related tokens. These evaluations provide insights into the model's biases by examining the likelihood of generating stereotype-associated content.

Several task-based benchmarks have been proposed to assess bias in LLMs. These include benchmarks for bias in text generation of letters of recommendation \cite{wan2023kelly}, bias in classification and prediction of gender in professional biographies \cite{De_Arteaga_2019}, and bias and stereotyping in question answering \cite{parrish2022bbq}. Additionally, the WinoBias benchmark \cite{zhao2018gender} measures gender bias in coreference resolution, serving as a clear example of an extrinsic evaluation.

\subsection{Language model biases evaluation across languages}

==> archive/4_logits_controlled_old.tex <==
%%%% Methods %%%%
\subsection{Methods}

\subsubsection{Experimental Framework}
We designed a controlled experimental framework to investigate model logit differences while only changing demographics or disease keywords. We created \textbf{10} templates, each engineered to incorporate a demographic relation and a disease term in various combinations. The templates aimed to state that a condition was common in a specific subgroup to evaluate the likelihood of that sentence occurring, such as \emph{Syphilis patients are usually Black}. To ensure robustness, we explored variations on these templates and evaluated both averages, ranks, and individual template results in Appendix \ref{template_robustness}.

\subsubsection{Model Selection}
We investigated the Hugging Face Pythia suite, which was trained on the deduplicated Pile dataset, and the Mamba suite, which was trained exclusively on the Pile dataset. This provides a controlled setting for evaluating logits with a fixed pretraining dataset and compares transformer-based and state space model architectures.

\subsubsection{Logit generation}
As described above, a unique sequence was passed into a specific model, and the logits were stored. \todo{should probably add a ref here for similar work} To evaluate the calibration of the models with real-world disease prevalences, particularly in the American context, we tested a variation of the templates that included the stem "for the American population." This generated a unique row for each unique combination, providing a disease demographic model logit dataset that could be mapped to the pretraining co-occurrences of the respective pairs. This joined dataset is available at \url{https://cross-care.vercel.app/downloads}.

\subsubsection{Exclusion of API-based models}
\todo{do we want to address API T/F logits at all - even state we tried but not reliable..? or move appendix?}
Due to the limitation of models accessed via APIs, where typically only the top 5 logits are returned, we evaluated a True logit approach. This method used the same templates but with an added stem requesting numeric values, then rephrasing True/False as 1/2. This approach enabled us to approximate the true logit values despite the API constraints. However, we compared the outputs to Huggingface-based models using the same T/F setup, but even with fixed temperatures, inconsistency among outputs prevents comparison with the sequence logit methods. They were, therefore, excluded from the remaining analysis.

\subsubsection{Aggregation and Ranking of Logits}
We generated logits for every template and calculated the mean logit score across the templates for each disease-demographic pair. We employed a rank-based approach, ranking the logit scores within each disease from highest to lowest within the demographic category (e.g., Asthma male/female/non-binary ranks 1/2/3).

\subsubsection{Comparative Analysis of Ranks}
We used the Kendall tau score to evaluate the rank generated by the logits within disease-demographic groups against a count rank generated using the same groups for co-occurrence counts. The Kendall taus were aggregated across diseases to assess the impact of co-occurrence. Additionally, we explored linear probes to predict disease logits from disease demographics, adding model size and type to assess their contribution to the model's bias.


%%%% Findings %%%%
\subsection{Findings}
%
%
\subsubsection{Race}
% Top
We observed notable variation across different models and model sizes in the accuracy of demographic ranking in Figure \ref{fig:controlled_race_top_rank_counts}. Black individuals were consistently ranked highly in the likelihood of disease across a wide range of conditions. Conversely, white individuals were also frequently mentioned, but there was limited mention of other minority groups. Overall, the correlation between co-occurrence rank matches and model logits for the highest ranking was generally poor.

% Bottom
In contrast, there was high agreement in the bottom rank counts, correctly placing Pacific islanders in the least likely category as shown in Figure \ref{fig:controlled_race_bottom_rank_counts}.

% 2nd Bottom
Examining the second-bottom counts shows a clear discrepancy in likelihood between the Hispanic and indigenous groups, shown in Figure \ref{fig:controlled_race_2_bottom_rank_counts}

% Top figure
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.49\textwidth}  % Specifies the subfigure size (49% of text width here)
        \centering
        \includegraphics[width=\textwidth]{images/pythia_top_race_count.png}  % Set image width relative to subfigure width
        \caption{Pythia.}  % Subcaption for the left image
        \label{fig:pythia_race_rank_stackplot}
    \end{subfigure}
    \hfill  % Adds horizontal space between the figures
    \begin{subfigure}{0.49\textwidth}  % Same width as the first subfigure
        \centering
        \includegraphics[width=\textwidth]{images/mamba_top_race_count.png}  % Same image as the left
        \caption{Mamba.}  % Subcaption for the right image
        \label{fig:mamba_race_rank_stackplot}
    \end{subfigure}
    \caption{Top ranked logits vs co-occurrences.}  % Main caption for the whole figure
    \label{fig:controlled_race_top_rank_counts}
\end{figure}
%
%
\subsubsection{Gender}
% Top
Regarding gender demographics, our results indicate similar variations across models and model sizes, Figure \ref{fig:controlled_gender_top_rank_counts}, however with a strong agreement for the least likely combination associated with non-binary in Figure \ref{fig:controlled_gender_bottom_rank_counts}.
% Top Gender figure
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.49\textwidth}  % Specifies the subfigure size (49% of text width here)
        \centering
        \includegraphics[width=\textwidth]{images/pythia_top_gender_count.png}  % Set image width relative to subfigure width
        \caption{Pythia.}  % Subcaption for the left image
        \label{fig:pythia_gender_rank_stackplot}
    \end{subfigure}
    \hfill  % Adds horizontal space between the figures
    \begin{subfigure}{0.49\textwidth}  % Same width as the first subfigure
        \centering
        \includegraphics[width=\textwidth]{images/mamba_top_gender_count.png}  % Same image as the left
        \caption{Mamba.}  % Subcaption for the right image
        \label{fig:mamba_gender_rank_stackplot}
    \end{subfigure}
    \caption{Top ranked logits vs co-occurrences.}  % Main caption for the whole figure
    \label{fig:controlled_gender_top_rank_counts}
\end{figure}
%
%
\subsubsection{Kendall Tau}
The Kendall Tau scores comparing the rankings of logits against real-world prevalence rankings were near zero across all model sizes, indicating no significant correlation for both race and gender (Figures \ref{fig:controlled_race_kt} and \ref{fig:controlled_gender_kt}. This suggests that the logit rankings of diseases by demographic groups within models do not align with their real-world prevalence rankings. However, there are differences between the models in how gender-related data is ranked, with some showing strong positive correlations.

% KT Race figure
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.49\textwidth}  % Specifies the subfigure size (49% of text width here)
        \centering
        \includegraphics[width=\textwidth]{images/race_pythia_pile_real_logits.png}  % Set image width relative to subfigure width
        \caption{Pythia.}  % Subcaption for the left image
        \label{fig:pythia_race_kt}
    \end{subfigure}
    \hfill  % Adds horizontal space between the figures
    \begin{subfigure}{0.49\textwidth}  % Same width as the first subfigure
        \centering
        \includegraphics[width=\textwidth]{images/race_mamba_pile_real_logits.png}  
        \caption{Mamba.}  % Subcaption for the right image
        \label{fig:mamba_race_kt}
    \end{subfigure}
    \caption{Top ranked logits vs co-occurrences.}  % Main caption for the whole figure
    \label{fig:controlled_race_kt}
\end{figure}

% KT gender figure
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.49\textwidth}  % Specifies the subfigure size (49% of text width here)
        \centering
        \includegraphics[width=\textwidth]{images/gender_pythia_pile_real_logits.png}  % Set image width relative to subfigure width
        \caption{Pythia.}  % Subcaption for the left image
        \label{fig:pythia_gender_kt}
    \end{subfigure}
    \hfill  % Adds horizontal space between the figures
    \begin{subfigure}{0.49\textwidth}  % Same width as the first subfigure
        \centering
        \includegraphics[width=\textwidth]{images/gender_mamba_pile_real_logits.png}  
        \caption{Mamba.}  % Subcaption for the right image
        \label{fig:mamba_gender_kt}
    \end{subfigure}
    \caption{Top ranked logits vs co-occurrences.}  % Main caption for the whole figure
    \label{fig:controlled_gender_kt}
\end{figure}

\subsubsection{Rank vs Mentions}
The analysis of Kendall Tau scores across quartiles of disease mentions in the Pile dataset reveals consistent relationships for both race (Figure \ref{fig:controlled_race_kt_quartile}) and gender (Figure \ref{fig:controlled_gender_kt_quartile}). Notably, the relationship between the frequency of disease mentions and the accuracy of logit correlations did not vary significantly across quartiles. This indicates that diseases most frequently mentioned in the dataset did not demonstrate a corresponding improvement in the correlation of logits, suggesting that model performance does not scale with the frequency of disease mention.

% KT Quartile Race figure
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.49\textwidth}  % Specifies the subfigure size (49% of text width here)
        \centering
        \includegraphics[width=\textwidth]{figures/4_pythia_kt_quartile_infinigram.png}  % Set image width relative to subfigure width
        \caption{Pythia.}  % Subcaption for the left image
        \label{fig:pythia_race_kt_quartile}
    \end{subfigure}
    \hfill  % Adds horizontal space between the figures
    \begin{subfigure}{0.49\textwidth}  % Same width as the first subfigure
        \centering
        \includegraphics[width=\textwidth]{figures/4_mamba_kt_quartile_infinigram.png}  
        \caption{Mamba.}  % Subcaption for the right image
        \label{fig:mamba_race_kt_quartile}
    \end{subfigure}
    \caption{KT quartile for race, infinigram.}  % Main caption for the whole figure
    \label{fig:controlled_race_kt_quartile}
\end{figure}


% Gender
% KT Quartile gender figure
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.49\textwidth}  % Specifies the subfigure size (49% of text width here)
        \centering
        \includegraphics[width=\textwidth]{figures/4_pythia_gender_kt_quartile_infinigram.png}  % Set image width relative to subfigure width
        \caption{Pythia.}  % Subcaption for the left image
        \label{fig:pythia_gender_kt_quartile}
    \end{subfigure}
    \hfill  % Adds horizontal space between the figures
    \begin{subfigure}{0.49\textwidth}  % Same width as the first subfigure
        \centering
        \includegraphics[width=\textwidth]{figures/4_mamba_gender_kt_quartile_infinigram.png}  
        \caption{Mamba.}  % Subcaption for the right image
        \label{fig:mamba_gender_kt_quartile}
    \end{subfigure}
    \caption{KT quartile for gender, infinigram.}  % Main caption for the whole figure
    \label{fig:controlled_gender_kt_quartile}
\end{figure}

\todo{decide if want to include infinigram vs. demographic counts for KT quartile and if want any in the appendix}

\subsection{Methods}

\subsubsection{Experimental Framework}
This section extends the work completed in the controlled setting using the same logit generation and evaluation framework. The same \textbf{10} templates used previously were employed here; however, the primary difference in template formatting includes adding a translation layer. We translated our templates, diseases, and demographic terms into English, Spanish, French, and Mandarin. Native speakers did this translation process to ensure accuracy and cultural relevance in the terms used.

\subsubsection{Model Selection}
For this study, we selected publicly available models that demonstrated variations in fine-tuning or continuous training settings, with an emphasis also on multilingual capabilities. The final set includes the LLama2, Qwen, and Mistral series from the 7B and 70B model sets.

\subsubsection{Aggregation and Ranking of Logits}
Logits for every translated template were generated and analyzed. We calculated the mean logit score across templates for each disease-demographic pair in each language, employing a rank-based approach as above to evaluate the logit scores within each disease from highest to lowest for each demographic category. Logits across languages were not aggregated at any point.

\subsection{Findings}

\subsubsection{Alignment across Fine-tuning strategies}

The impact of different fine-tuning strategies on the LLama series for both race and gender are displayed in Figures \ref{fig:llama_race_stack} and \ref{fig:llama_gender_stack}. 

Comparisons across the Qwen and Mistral series are presented in the Appendix in Figures \ref{fig:qwen_race_stack}, \ref{fig:mistral_race_stack}, \ref{fig:qwen_gender_stack}, and \ref{fig:mistral_gender_stack}.

% LLama Race
\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{images/race_rlfh_70b_llama_top_count_distribution.png}  % Set image width relative to subfigure width
    \caption{Llama series Race.}  % Subcaption for the left image
    \label{fig:llama_race_stack}
\end{figure}

% LLama Gender
\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{images/gender_rlfh_70b_llama_top_count_distribution.png}  % Set image width relative to subfigure width
    \caption{Llama series Gender.}  % Subcaption for the left image
    \label{fig:llama_gender_stack}
\end{figure}

\todo{we need to decide whether we put table under figure across languages as ppt or split into two- have a figure, then table for english only race + gender, then a table for llama just race across languages, etc.}

% English only table alignment
The change in top counts and their subsequent impact on the Kendall tau between model logit ranking and the real-world prevalence can be seen in Table \ref{tab:llama_alignment_en}
\input{tables/5_llama_alignment}

\subsubsection{Impact of Fine tuning strategies on Alignment across Languages}
\input{tables/5_llama_race_alignment}

Language impact on qwen and mistral can be found in Tables  



KT are presented in the tables above. 
\todo{consider if want to add the line chart too for KT in the wild vs table only} 

